Semantic-aware Sampling and Transmission in Energy Harvesting Systems: A POMDP Approach

We address the problem of real-time remote tracking of a partially observable Markov source in an energy harvesting system with an unreliable communication channel. We consider both sampling and transmission costs. Different from most prior studies that assume the source is fully observable, the sampling cost renders the source partially observable. The goal is to jointly optimize sampling and transmission policies for two semantic-aware metrics: i) a general distortion measure and ii) the age of incorrect information (AoII). We formulate a stochastic control problem. To solve the problem for each metric, we cast a partially observable Markov decision process (POMDP), which is transformed into a belief MDP. Then, for both AoII under the perfect channel setup and distortion, we express the belief as a function of the age of information (AoI). This expression enables us to effectively truncate the corresponding belief space and formulate a finite-state MDP problem, which is solved using the relative value iteration algorithm. For the AoII metric in the general setup, a deep reinforcement learning policy is proposed to solve the belief MDP problem. Simulation results show the effectiveness of the derived policies and, in particular, reveal a non-monotonic switching-type structure of the real-time optimal policy with respect to AoI.

==> Chapters/backuptext.tex <==
Introduction:

+++++++

is controllable and it can generate a sample upon a (sampling) command. The transmitter then transmit the sample if there is mismatch between the source state and destination. 
Each sampling and transmission, respectively, incur different sampling cost and transmission cost in terms of energy usage. As the harvested energy is only the source of energy, this induce a per-slot, so-called energy causality constraint. 

We formulate a stochastic (control) optimization problem aiming at to minimize a semantic-aware metric  subject to energy causality constraint; specifically, we study the AoII, MSE, and AoI. 
It is evident that each of these metrics will necessitate different modeling and design approaches.
For each of the metrics,  the optimization problem is cast into MDP and POMDP problem. Then, by verifying the technical conditions of the underlying MDP/POMDP framework, 
 we derive an optimal policy for each of the three metrics.  
 By characterizing the belief space in casting the POMDP problems for the AoII and MSE, we obtain  MDP problems whose objective is a non-linear function of the AoI.  
 Extensive simulation results are conducted to compare  the performance of the different metrics, and show the effectiveness of the polices. 
 As a main results, simulation results shows that a MSE-optimal policy is also optimize average AoII in the considered system.



Timely delivery of status updates of a remotely monitored process to a destination is needed to support the emerging time-critical applications in the future Internet of things (IoT) in 5G and 6G wireless generations, e.g., industrial control, smart home systems, and drone control.
The age of information (AoI) is initially introduced to capture/quantify the freshness of information \cite{Roy_2012}. 
Nowdays, there are significant research on the AoI in different areas, e.g., queuing system \cite{Marian_Information}, and  scheduling and sampling problems \cite{Zakeri_Journal_Relay, Eyton_Modiano}. 
However, it has been confirmed in, e.g., \cite{Tony_1}, that the AoI may be inefficient in capturing the freshness, as it is essentially blind to  what information/message/goal is being carried by the status updates. This motivated a different research direction, so-called beyond AoI, which led to the idea of  using, e.g., 
%non-linear AoI \cite{Sun_1}, the value of information \cite{},
the age of incorrect information (AoII) \cite{Tony_1} and mean squared error (MSE) \cite{Yin_Sun_EstAcm} to capture the freshness. 

Both the AoII and MSE incorporate, in the core,  the source's information and its knowledge at the (remote) monitor side called  the \textit{estimation} of the source at the monitor. To that extent, we should note that the MSE here is a distortion metric and captures a difference between the state of a source of information and its estimation at the monitor, not the quality of the estimation; thus, it can be equivalent to  
the actuation error cost in \cite{Nikolaos_goal_or}, which considers a (state-estimation-dependent) cost when there is an error between the source and the estimation. 
Accordingly, both AoII and MSE take into account the semantic of information in terms of contextual importance (or goal) of transmitted information\cite{Nikolaos_goal_or,}.

To optimize the real-time error and the AoII, the knowledge of the source state and the estimation required, which entails continues sampling (and processing) of the underlying source process.\footnote{
Say about the sampling meaning difference here \cite{Kam_2018}.
}
The practical limitations of this are such that it incurs constant sampling costs, or may even be impossible to sample due to insufficient energy, as is often the case in energy harvesting systems. 
However, in most of recent works, e.g., \cite{Kam_2018,Tony_1, Nikolaos_goal_or}, considered the source state is always observable (by the controller), and,
to the best of our knowledge, only work \cite{Niko_DistortionSampCost} considered a sampling cost. 

At the same time, in many IoT applications, the devices are typically not supplied with a power source and instead rely on irreplaceable batteries (with limited life time). Consequently, energy harvesting solutions are often the most effective and feasible means of powering these devices, with harvested energy serving as the sole source for both sampling and transmission. As a result, designing sampling and scheduling policies imposes significant challenges that require careful consideration of energy arrivals and usage due to the intermittent nature of energy availability.

 
% =========================
%---
%Motivating by this, some another new (and related to the AoI) metrics are introduced, e.g., the age of incorrect information (AoII) \cite{Tony_1}, and the  mean squared error (MSE) \cite{Yin_Sun_EstAcm} to capture the freshness
%----
% \blue{
% In wireless communication networks, the age of information (AoI) has emerged as a metric to quantify the freshness of information at a monitoring node. The AoI reflects the time elapsed since the most recently received correct information at the monitoring node. However, it is assumed that the last received information is always correct, which is not necessarily the case in many real-time monitoring systems. To address this limitation, the age of incorrect information (AoII) has been proposed as a complementary metric to the AoI. The AoII is defined as the time elapsed since the last received incorrect information between the source and the monitoring node. This metric provides a more accurate measure of the freshness of information and can play a critical role in systems where the cost of acting upon outdated or incorrect information can be substantial. In this introduction, we will explore the concept of AoII, its applications, and the key technologies that enable its implementation. We will also examine the challenges and opportunities presented by this metric and its potential impact on the design of future real-time monitoring systems.}

Motivated by two practical consideration that: 1) the sampling cost that renders the source non-observable, and 2) the dependence on harvested energy as the sole source of power, we aim to find optimal semantic-aware joint sampling and scheduling policies in an energy-harvesting remote tracking system. Particularly, we consider a remote tracking system consisting of a paired source and monitor, as depicted in Fig. \ref{Fig_EnrHar}. The sampler is controllable and it can generate a sample upon a (sampling) command. The transmitter then transmit the sample if there is mismatch between the source state and destination. 
Each sampling and transmission, respectively, incur different sampling cost and transmission cost in terms of energy usage. As the harvested energy is only the source of energy, this induce a per-slot, so-called energy causality constraint. 

We formulate a stochastic (control) optimization problem aiming at to minimize a semantic-aware metric  subject to energy causality constraint; specifically, we study the AoII, MSE, and AoI. 
It is evident that each of these metrics will necessitate different modeling and design approaches.
For each of the metrics,  the optimization problem is cast into MDP and POMDP problem. Then, by verifying the technical conditions of the underlying MDP/POMDP framework, 
 we derive an optimal policy for each of the three metrics.  
 By characterizing the belief space in casting the POMDP problems for the AoII and MSE, we obtain  MDP problems whose objective is a non-linear function of the AoI.  
 Extensive simulation results are conducted to compare  the performance of the different metrics, and show the effectiveness of the polices. 
 As a main results, simulation results shows that a MSE-optimal policy is also optimize average AoII in the considered system.

